Expanding Pretrained Models to Thousands More Languages via Lexicon-based Adaptation

The performance of multilingual pretrained models is highly dependent on the availability of monolingual or parallel text present in a target language. Thus, the majority of the world's languages cannot benefit from recent progress in NLP as they have no or limited textual data. To expand possibilities of using NLP technology in these under-represented languages, we systematically study strategies that relax the reliance on conventional language resources through the use of bilingual lexicons, an alternative resource with much better language coverage. We analyze different strategies to synthesize textual or labeled data using lexicons, and how this data can be combined with monolingual or parallel text when available. For 19 under-represented languages across 3 tasks, our methods lead to consistent improvements of up to 5 and 15 points with and without extra monolingual text respectively. Overall, our study highlights how NLP methods can be adapted to thousands more languages that are under-served by current technology

==> method_deprecated.tex <==
%\section{Languages with Limited Resources}
\section{Background}
\subsection{Conventional Adaptation Data}
First we introduce two widely adopted paradigms for adapting these models to a target language using monolingual or parallel data.

\paragraph{Monlingual Data} Continued pretraining on monolingual data related to the downstream task is shown to be effective at improving the performance of English pretrained model~\citep{dont-stop-pretrain-gururangan-etal-2020}. \citep{muller-etal-2021-unseen} find that continue pretraining the multilingual models on \textit{monolingual data} of the target language can effectively adapt the model to the target language. Notably, \citep{adapt-1600-languages} show that using as little as several thousand monolingual sentences in the target language can significantly improve the pretrained multilingual model's performance on languages that are not covered during pretraining.   

\paragraph{Parallel Data} For target languages with \textit{parallel data} between English available, one could train a good NMT system that translates from English into the target language. Using such an NMT system, we can translate the English task data into the target language, and finetune the pretrained multilingual model on both the English and translated task data. This method can often bring significant gains to the target language, especially for the languages with high-quality NMT systems~\citep{xtreme}.

\subsection{Low-resource Languages}
\citet{joshi-etal-2020-state} classified the 7000 languages of the World into 6 groups based on the availability of data where each group follows a different trajectory of NLP development. Two of the six groups face the biggest challenges in having competitive NLP tools despite having the largest percentage of language varieties:
\begin{itemize}
    \item  ``The Left-Behinds'' are languages with virtually no unlabeled data. We use ``No-Text'' to refer to this group.
    \item ``The Scraping-Bys'' are languages with a small amount of monolingual data. We use ``Few-Text'' to refer to this group.
\end{itemize}
These two groups take up more than $85\%$ of languages of the World, yet they cannot benefit from the development of pretrained models and adaptation methods due to the lack of monolingual and parallel data~\citep{joshi-etal-2020-state}. In this paper, we conduct systematic study of the resource and methods we can leverage to ``lift up'' these two groups of languages.      


\section{Adapting to No-Text and Few-Text}
Since the main bottleneck of these low-resource languages is the lack of monolingual and parallel data, two natural question arises: are there any alternative resources we can leverage to synthesize data into the two groups of low-resource languages, and how can we utilize the limited data when available? In this section, we outline a data augmentation framework~(illustrated in \autoref{fig:method}) that addresses the two questions.

\subsection{Sythesizing Data Using Lexicons}
PanLex\footnote{\url{https://panlex.org/}} is a non-profit project that aims to collect lexicons for every language variety in the world. Currently it covers over 5000 language varieties, offering much wider coverage than Wikipedia and the Bible. Given a bilingual lexicon between English and a target language $T$, we can create synthetic sentences in $T$ using English data by word-to-word translation.

\paragraph{Pseudo Monolingual Data} Given monolingual English data, we can generate pseudo monolingual data for $T$ by word-to-word with a lexicon. Similar to continued MLM using real monolingual data in the language $T$, we can adapt the pretrained multilingual model on the pseudo monolingual data using the MLM objective.

\paragraph{Pseudo Task Data} Given the English task data pairs $\langle x, y \rangle$, we use the lexicon to replace the words in $x$ into its corresponding translation in $T$, resulting in pseudo task data $\langle x_t, y \rangle$. Then we can finetune the model jointly on both $\langle x, y \rangle$ and $\langle x_t, y \rangle$.

Since these methods only require bilingual lexicons, we can apply them to both groups of languages. We can use either of the two methods to adapt a baseline model or the combination of both.  

\paragraph{Label Distillation} 
The pseudo task data contain label noise because the pseudo source $x_t$ might have a different label in the target language, yet we simply keep the original label $y$ in English. To alleviate this issue, we propose to automatically ``correct'' the labels of pseudo task data using a teacher model. Specifically, we finetune the pretrained multilingual model using only English task data as the teacher model, which is used to generate label $y_t$ for the pseudo task input $x_t$. 
Then we finetune the pretrained model again on both the pseudo data $\langle x_t, y_t \rangle$ and the English task data $\langle x, y \rangle$.

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{plots/pseudo_icons_crop.pdf}
    \caption{Pipelines for synthesizing data for the \textcolor{blue}{two language groups} and utilizing data for the \textcolor{brown}{Few-Text}. We can use either Pseudo MLM or Pseudo Fine-tune, or both.}
    %\sr{This diagram looks great already. Could you also add circles representing the English monolingual and English task data? I think incorporating these would make clearer what types of data are necessary for generating the different resources.}}
    \label{fig:method}
\end{figure}
\subsection{Efficiently Utilize data for Few-Text}
Languages in the Few-Text group generally have small amount of monolingual or parallel data available, which we can utilize to further boost their performance.
\paragraph{Monolingual Data} We can train the model jointly on the pseudo monolingual data and the gold monolingual data using the MLM objective.
\paragraph{Parallel Data} Since the parallel data in these languages usually only contain very limited sentences from a constraint domain such as the Bible, we cannot use them to train as good NMT systems as the high-resource languages~(we verify this in \autoref{sec:nmt}). Therefore, we propose to induce additional lexicons from the parallel data using unsupervised word alignment. Adding these entries to the original lexicons can potentially boost word coverage and improve the quality of the synthetic data.

==> method_old.tex <==
%\section{Languages with Limited Resources}
\section{Background}
\subsection{Existing Adaptation Methods}
First we introduce two widely adopted paradigms for adapting these models to a target language using monolingual or parallel data.

\paragraph{Monlingual Data} Continued pretraining on monolingual data related to the downstream task is shown to be effective at improving the performance of English pretrained model~\citep{dont-stop-pretrain-gururangan-etal-2020}. \citep{muller-etal-2021-unseen} find that continue pretraining the multilingual models on \textit{monolingual data} of the target language can effectively adapt the model to the target language. Notably, \citep{adapt-1600-languages} show that using as little as several thousand monolingual sentences in the target language can significantly improve the pretrained multilingual model's performance on languages that are not covered during pretraining.   

\paragraph{Parallel Data} For target languages with \textit{parallel data} between English available, one may have access to a good NMT system that translates from English into the target language. Using such an NMT system, we can translate the English task data into the target language, and finetune the pretrained multilingual model on both the English and translated task data. This method can often bring significant gains to the target language, especially for the languages with high-quality NMT systems~\citep{xtreme}.

\subsection{Low-resource Languages}
\citet{joshi-etal-2020-state} classified the 7000 languages of the World into 6 groups based on the availability of data where each group follows a different trajectory of NLP development. Two of the six groups face especially great challenges in having competitive NLP tools despite having the largest percentage of language varieties:
\begin{enumerate}
    \item  ``The Left-Behinds'' are languages with virtually no unlabeled data.
    \item ``The Scraping-Bys'' are languages with a small amount of monolingual data.
\end{enumerate}
These two groups take up more than $85\%$ of languages of the World, yet they cannot benefit from the development of pretrained models and adaptation methods due to the lack of monolingual and parallel data. In this paper, we conduct systematic study of the resource and methods we can leverage to ``lift up'' these two groups of languages.      

\section{Adapting to the Left-Behinds and the Scraping-Bys}
Despite the effectiveness of the two adaptation paradigms, they are both constraint by the availability of monolingual and parallel data in the target language. As \autoref{fig:languages} shows, about $20\%$ of world's languages have only limited monolingual data and over $70\%$ of the languages do not have any monolingual data available.
A natural question arises: can we design a method to synthesize data into the low-resourced target languages so that we can apply these two paradigms? In this section, we lay out such a data augmentation strategy for extremely low-resourced languages. 
\subsection{Utilizing Existing Resources}
Although many languages lack easily accessible monolingual and parallel data due to the limited usage on the Internet, there might be other types of data in these languages we can leverage. For example, there are many efforts in documenting languages through lexicons and word lists~\citep{}. We argue that it is essential to examine and utilize these existing linguistic resources to train and adapt competitive NLP models that benefit speakers of the next thousands of languages. In this paper, we provide a case study on using lexicons for this purpose.

\paragraph{Sythesizing Data Using Lexicons} PanLex\footnote{\url{https://panlex.org/}} is a non-profit project that aims to collect lexicons for every language variety in the world. Currently it covers over 5000 language varieties, offering much wider coverage than Wikipedia and the Bible. Given a lexicon extracted from PanLex between English and a target language $T$, we can create synthetic sentences in $T$ using English data by word-to-word translation. Next we outline two strategies that adapt pretrained multilingual models to a target language with the synthetic data.

\subsection{Adaptation Methods}

\paragraph{Pseudo MLM} Given monolingual English data, we can generate pseudo monolingual data for $T$ by word-to-word with a lexicon. Similar to continued MLM using real monolingual data in the language $T$, we can adapt the pretrained multilingual model on the pseudo monolingual data using the MLM objective.

\paragraph{Pseudo Finetune} Given the English task data pairs $\langle x, y \rangle$, we use the lexicon to replace the words in $x$ into its corresponding translation in $T$, resulting in pseudo task data $\langle x_t, y \rangle$. Then we can finetune the model jointly on both $\langle x, y \rangle$ and $\langle x_t, y \rangle$.

Note that these methods only require a lexicon between English and $T$, so we can apply them to languages without any monolingual data or those with a little monolingual data available. We can use either of the two methods to adapt a baseline model, or combining both by doing Pseudo Finetune on top of a model adapted with Pseudo MLM.  
%In the next section, we outline a comprehensive comparison of different adaptation strategies using synthetic data under settings where one has no monolingual data or has access to some monolingual data in the target language.


